Coding for Caches in the Plane

We consider wireless caches located in the plane according to general point process and specialize the results for the homogeneous Poisson process. A large data file is stored at the caches, which have limited storage capabilities. Hence, they can only store parts of the data. Clients can contact the caches to retrieve the data. We compare the expected cost of obtaining the complete data under uncoded as well as coded data allocation strategies. It is shown that for the general class of cost measures where the cost of retrieving data is increasing with the distance between client and caches, coded allocation outperforms uncoded allocation. The improvement offered by coding is quantified for two more specific classes of performance measures. Finally, our results are validated by computing the costs of the allocation strategies for the case that caches coincide with currently deployed mobile base stations.

==> plotw.tex <==
% This file was created by matlab2tikz v0.3.3.
% Copyright (c) 2008--2013, Nico Schlmer <nico.schloemer@gmail.com>
% All rights reserved.
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
% 
% 

% defining custom colors
\definecolor{mycolor1}{rgb}{1,0,1}

\begin{tikzpicture}
\pgfplotsset{compat=1.3}
\begin{axis}[%
width=.7\linewidth,
height=.5\linewidth,
scale only axis,
xmin=1,
xmax=5,
ymin=0,
ymax=150,
xlabel={$k$},
ylabel={$W$},
ylabel style={rotate=-90}, %at={(ticklabel cs:0.7)}
legend style={draw=black,fill=white,legend cell align=left, font=\small},
tick label style={font=\small},
label style={font=\small},
line width = 1pt
]
\addplot [
color=blue,
solid
]
table[row sep=crcr]{
1 2.51646060522626\\
2 14.2352711182479\\
3 39.2319924074385\\
4 80.5772135950175\\
5 140.809863948231\\
};
\addlegendentry{$W^p$};

\addplot [
color=red,
solid
]
table[row sep=crcr]{
1 2.51646060522626\\
2 6.2911515131245\\
3 11.0095151489213\\
4 16.5142727336869\\
5 22.7071250924389\\
};
\addlegendentry{$W^c_\mathrm{min}$};


\addplot [
color=mycolor1,
solid
]
table[row sep=crcr]{
1 2.90708560522626\\
2 7.850599755312\\
3 14.5114251201584\\
4 22.7277469142363\\
5 32.3967535887284\\
};
\addlegendentry{$W^c_\mathrm{min}+W_0$};

\end{axis}
\end{tikzpicture}%
